Exploring the AGN-ram pressure stripping connection in local clusters

Ram-pressure stripping by the intracluster medium (ICM) is one of the most advocated mechanisms that affect the properties of cluster galaxies. A recent study based on a small sample has found that many galaxies showing strong signatures of ram-pressure stripping also possess an active galactic nucleus (AGN), suggesting a possible correlation between the two phenomena. This result has not been confirmed by a subsequent study. Building upon previous findings, here we combine MUSE observations conducted within the GASP program and a general survey of the literature to robustly measure the AGN fraction in cluster's ram pressure stripped galaxies using BPT emission line diagrams. Considering a sample of 115 ram pressure stripped galaxies with stellar masses $\geq 10^9 \, M_{\odot}$, we find an AGN fraction of $\sim27\%$. This fraction strongly depends on stellar mass: it raises to 51% when only ram-pressure stripped galaxies of masses $M_* \geq 10^{10} \, M_{\odot}$ are considered. We then investigate whether the AGN incidence is in excess in ram pressure stripped galaxies compared to non-stripped galaxies, using as comparison a sample of non-cluster galaxies observed by the survey MaNGA. Considering mass-matched samples, we find that the incidence of AGN activity is significantly higher (at a confidence level $>99.95\%$) when ram-pressure stripping is on act, supporting the hypothesis of an AGN-ram pressure connection.

==> AASTeX Template for submissions to AAS Journals (ApJ-AJ-ApJS-ApJL-PSJ-RN) (2) (4)/table3_ALL_revised.tex <==
\begin{longrotatetable}
\begin{deluxetable}{ccccccccc}
\tabletypesize{\tiny}
\tablecaption{Colums are: 1) name 2) and 3) equatorial coordinates of the galaxy center from SIMBAD 4) galaxy redshift 5) host cluster 6) and 7) Jstage and general Jstage, defined in section \S3.2 8) alternative names and authors from which information have been taken. Stellar masses flagged with the asterisk (*) are computed by means of photometric data as described in Sec.\ref{sec:appendix_mass}. 
\label{litt_sample}}
\tablehead{
  \colhead{name} &
  \colhead{RA} &
  \colhead{DEC} &
  \colhead{z} &
  \colhead{cluster} &
  \colhead{Jstage} &
  \colhead{Jstage$_{\rm gen}$} &
  \colhead{comments}
 }
 \tablewidth{0pt}
  \startdata
\hline
  MIP001417-302303 & 3.5693 & -30.3843 & 0.2955 & A2744 & -- & 2.0 & F1228\\
  HLS001427-302344 & 3.61065 & -30.39581 & 0.3033 & A2744 & -- & 2.0 & F0083\\
  NGC1566 & 65.00175 & -54.93781 & 0.005 & Dorado & 0.0 & 0.0 & --\\
  ID345 & 149.9191 & 2.5281 & 0.727 & CGr32 & 2.0 & 2.0 & --\\
  LEDA36382 & 175.73523 & 19.96621 & 0.02427 & A1367 & 2.0 & 2.0 & CGCG97073\\
  UGC6697 & 175.95446 & 19.96844 & 0.02243 & A1367 & 2.0 & 2.0 & CGCG097-087\\
  2MASXJ11443212+2006238 & 176.13385 & 20.10662 & 0.02398 & A1367 & 2.0 & 2.0 & --\\
  NGC4254 & 184.70668 & 14.41651 & 0.00803 & Virgo & 1.0 & 2.0 & MESSIER099\\
  NGC4388 & 186.44508 & 12.66207 & 0.00856 & Virgo & 1.0 & 2.0 & UGC07520, VCC 0836, VPC 0438, CGCG070068\\
  NGC4402 & 186.53189 & 13.11332 & 0.0008   & Virgo & 3.0 & 0.5 &   VCC873\\    
  NGC4424 & 186.79838 & 9.42067  & 0.0015 & Virgo & 0.5 & 2             & -- \\
  NGC4438 & 186.93997 & 13.00883 & 0.0003 & Virgo & -- & -- & --\\
  IC3418 & 187.43301 & 11.40469 & 0.00013 & Virgo & 0.5 & 2.0 & VCC1217\\
  NGC4501 & 187.9965 & 14.42039 & 0.00761 & Virgo & -- & 0.5 & MESSIER088\\
  NGC4522 & 188.41546 & 9.17502 & 0.0077 & Virgo & 3.0 & 1.0 & --\\
  NGC4548 & 188.86022 & 14.49634 & 0.00164 & Virgo & 0.0 & 0.0 & MESSIER091\\
  NGC4569 & 189.20747 & 13.16294 & 0.0008.0 & Virgo & 2.0 & 2.0 & MESSIER090, UGC07786, VCC 1690\\
  GMP6364 & 193.67526 & 27.63897 & 0.02874 & Coma & -- & 2.0 & SDSS J125442.05+273820.2\\
  GMP5821 & 193.93454 & 28.75464 & 0.0275 & Coma & -- & -- & SDSS J125544.29+284516.6\\
  IC3913 & 194.11905 & 27.29128 & 0.0251 & Coma & -- & -- & GMP5422, KUG 1254+275, CGCG160026\\
  GMP5382 & 194.11967 & 29.13708 & 0.03163 & Coma & -- & 0.0 & 2MASX J12562871+2908140, SDSS J125628.71+290813.5\\
  GMP4688 & 194.43215 & 29.00331 & 0.0231 & Coma & -- & 1.0 & LEDA 1852727\\
  GMP4629 & 194.4593 & 28.17036 & 0.0231 & Coma & 1.0 & 1.0 & SDSSJ125750.2+281013\\
  GMP4570 & 194.48665 & 27.99176 & 0.0152 & Coma & 2.0 & 2.0 & SDSSJ125756.79+275930\\
  GMP4555 & 194.4905 & 28.06178 & 0.0271 & Coma & 2.0 & 2.0 & SDSSJ125757.7+280342, KUG1255+283\\
  MACSJ1258-JFG1 & 194.49833 & 47.0461 & 0.3424 & MACSJ1258.0+4702 & -- & 2.0 & --\\
  NGC4848 & 194.52352 & 28.24274 & 0.0314 & Coma & 2.0 & 2.0 & GMP4471, CGCG 160-055, SDSSJ125805.6+281433, UGC08082, KUG 1255+285\\
  GMP4437 & 194.53846 & 28.70859 & 0.0254 & Coma & -- & 0.0 & --\\
  GMP4463 & 194.53858 & 26.66409 & 0.0243 & Coma & -- & 0.0 & --\\
  GMP4281 & 194.60575 & 28.12897 & 0.0274 & Coma & -- & 0.0 & --\\
  GMP4236 & 194.6285 & 26.99494 & 0.0249 & Coma & -- & 1.0 & --\\
  NGC4853 & 194.64663 & 27.59633 & 0.0256 & Coma & 0.0 & 0.0 & --\\
  GMP4159 & 194.64717 & 27.26486 & 0.0245 & Coma & -- & 0.5 & SDSSJ125835.2+273547, GMP4156, CGCG160068,  UGC08092, KUG1256+278B, D43\\
  GMP4135 & 194.65538 & 27.17625 & 0.0256 & Coma & -- & 1.0 & Mrk 56, KUG1256+27\\
  GMP4106 & 194.66637 & 26.7595 & 0.0249 & Coma & -- & 1.0 & Mrk057, KUG1256+274\\
  IC3949 & 194.73338 & 27.83336 & 0.0253 & Coma & 1.0 & 1.0 & --\\
  NGC4858 & 194.7585 & 28.11575 & 0.0314 & Coma & 2.0 & 2.0 &  SDSSJ125856.0+275000, GMP3896, CGCG160212, UGC08096, D89\\
  Mrk58 & 194.772 & 27.64446 & 0.0181 & Coma & 2.0 & 2.0 & GMP3816, SDSSJ125902.0+280656, CGCG160213, KUG1256+283\\
  GMP3618 & 194.81937 & 27.10608 & 0.028 & Coma & -- & 0.5 & GMP3779, KUG1256+279, CGCG160073, SDSSJ125905.2+27383840, D54, RB219\\
  GMP3271 & 194.91621 & 27.57625 & 0.0167 & Coma & 0.5 & 1.0 & --\\
  GMP3253 & 194.91721 & 28.63081 & 0.0178 & Coma & -- & 0.5 & D41, SDSSJ125939.8+273435, KUG1257+278\\
  GMP3143 & 194.95524 & 26.97433 & 0.0235 & Coma & -- & 0.0 & KUG 1257+288B\\
  GMP3071 & 194.9838 & 27.74633 & 0.0298 & Coma & 2.0 & 2.0 & --\\
  SDSSJ130006.15+281507.8 & 195.02568 & 28.25234 & 0.0212 & Coma & -- & 2.0 & --\\
  D100 & 195.03809 & 27.86649 & 0.0177 & Coma & 2.0 & 2.0 & Mrk60, GMP2910\\
  GMP2625 & 195.13003 & 28.95054 & 0.0233 & Coma & -- & 0.5 & --\\
  GMP2599 & 195.14031 & 27.63777 & 0.025 & Coma & 0.0 & 1.0 & --\\
  IC4040 & 195.15777 & 28.05809 & 0.0255 & Coma & 2.0 & 2.0 & KUG1258+279A, 7W 1258+27W06\\
  NGC4911 & 195.23357 & 27.79087 & 0.0266 & Coma & 1.0 & 1.0 & --\\
  GMP2073 & 195.35448 & 28.67723 & 0.0292 & Coma & -- & 0.0 & GMP2374\\
  NGC4921 & 195.35884 & 27.886 & 0.0183 & Coma & 0.0 & 0.0 & --\\
  GMP1616 & 195.53284 & 27.64831 & 0.023 & Coma & -- & 0.0 & GMP2059\\
  GMP1582 & 195.54739 & 28.17326 & 0.0299 & Coma & -- & 0.0 & --\\
  GMP713 & 195.97679 & 28.31054 & 0.0268 & Coma & -- & -- & LEDA 83761\\
  GMP672 & 195.98809 & 26.72948 & 0.022 & Coma & -- & 1.0 & --\\
  GMP597 & 196.0547 & 28.54245 & 0.0271 & Coma & -- & 0.5 & --\\
  GMP522 & 196.09452 & 28.81077 & 0.0265 & Coma & -- & 1.0 & --\\
  GMP455 & 196.11063 & 27.30431 & 0.0184 & Coma & -- & 2.0 & --\\
  GMP406 & 196.16159 & 28.97269 & 0.0253 & Coma & -- & 0.0 & --\\
  GMP223 & 196.27764 & 28.64115 & 0.0182 & Coma & -- & 1.0 & --\\
  SDSSJ130545.34+285216.8 & 196.439 & 28.87133 & 0.0266 & Coma & -- & 1.0 & --\\
  SDSSJ130553.48+280644.7 & 196.47287 & 28.11244 & 0.0246 & Coma & -- & 0.0 & --\\
  JO147 & 201.707304 & -31.39575 & 0.0506 & A3558 & 2.0 & 2.0 & SOS114372\\
  SOS90630 & 202.368875 & -31.657111 & 0.049 & SC1327-312 & 2.0 & 2.0 & --\\
  SOS61086 & 202.999167 & -31.822833 & 0.045 & SC1329-313 & 2.0 & 2.0 & --\\
  d4 & 203.135758 & 50.564581 & 0.272 & A1758 & -- & 0.5 & --\\
  A1758N\_JFG1 & 203.146583 & 50.52675 & 0.2733 & A1758 & 0.0 & 1.0 & --\\
  d5 & 203.17445 & 50.525994 & 0.2716 & A1758 & -- & 0.5 & --\\
  d7 & 203.184258 & 50.518794 & 0.2875 & A1758 & -- & 0.0 & --\\
  d6 & 203.1906 & 50.527164 & 0.2668 & A1758 & -- & 0.5 & --\\
  d3 & 203.208908 & 50.555894 & 0.2755 & A1758 & -- & 1.0 & --\\
  d1 & 203.224104 & 50.526292 & 0.2686 & A1758 & -- & 2.0 & --\\
  d2 & 203.226979 & 50.516425 & 0.2719 & A1758 & -- & 1.0 & --\\
  C153 & 235.2875 & 66.26222 & 0.2525 & A2125 & -- & 1.0 & --\\
  ESO137-001 & 243.363771 & -60.764053 & 0.01557 & A3627 & 2.0 & 2.0 & --\\
  ESO137-002 & 243.398546 & -60.865167 & 0.0191 & A3627 & 2.0 & 2.0 & --\\
  Sausage9 & 340.671125 & 52.974631 & 0.1839 & CIZAJ2242.8+5301 & -- & -- & --\\
  Sausage7 & 340.740125 & 53.087431 & 0.1832 & CIZAJ2242.8+5301 & -- & -- & --\\
  Sausage6 & 340.749375 & 53.037381 & 0.1836 & CIZAJ2242.8+5301 & -- & -- & --\\
  Sausage8 & 340.787 & 53.090289 & 0.1843 & CIZAJ2242.8+5301 & -- & -- & --\\
  Sausage5 & 340.80375 & 53.0028 & 0.1825 & CIZAJ2242.8+5301 & -- & -- & --\\
  235144-260358 & 357.933458 & -26.066555 & 0.2265 & A2667 & -- & 2.0 & --\\
\enddata
\end{deluxetable}
\end{longrotatetable}




==> AASTeX Template for submissions to AAS Journals (ApJ-AJ-ApJS-ApJL-PSJ-RN) (2) (4)/table3_short.tex <==


\begin{table*}
\begin{center}
\caption{Colums are: 1) galaxy most common name 2) and 3) equatorial coordinates of the galaxy center from SIMBAD 4) galaxy redshift 5) host cluster 6) and 7) Jstage and general Jstage, defined in section \S3.2 8) alternative names. % and authors from which information have been taken. 
Stellar masses flagged with the asterisk (*) are computed by means of photometric data as described in Sec.\ref{sec:appendix_mass}. \label{litt_sample}} 
\scriptsize
\begin{tabular}{cccccccc}
\hline
\hline
name & RA & DEC & z & cluster & Jstage   &Jstage$_{\rm gen}$ & alternative names \\
\hline
  MIP001417-302303 & 3.5693 & -30.3843 & 0.2955 & A2744 & -- & 2.0 & F1228\\
  HLS001427-302344 & 3.61065 & -30.39581 & 0.3033 & A2744 & -- & 2.0 & F0083\\
  NGC1566 & 65.00175 & -54.93781 & 0.005 & Dorado & 0.0 & 0.0 & --\\
  ID345 & 149.9191 & 2.5281 & 0.727 & CGr32 & 2.0 & 2.0 & --\\
  LEDA36382 & 175.73523 & 19.96621 & 0.02427 & A1367 & 2.0 & 2.0 & CGCG97073\\
\hline
\end{tabular}%
\end{center}
\tablecomments{This table is published in its entirety in machine-readable format.  A portion is shown here for guidance regarding its form and content.}\end{table*}


==> AASTeX Template for submissions to AAS Journals (ApJ-AJ-ApJS-ApJL-PSJ-RN) (2) (4)/table4_ALL_revised.tex <==



\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\startlongtable
\begin{deluxetable*}{lP{4cm}P{4cm}P{4cm}}
\tablecaption{Columns are 1) galaxy most common name 2) logarithm of the stellar masses, homogenizing them to our adopted Chabrier IMF (in parenthesis the reference from which the value has been taken is reported) 3) AGN classification (see Table \ref{gasp_agn}) and relative reference 4) references which present a characterization of the galaxy as a RPS candidate. The four galaxies with classification equals to 4 and 5 (e.g. where the AGN is spotted observing them in X and radio) resulted to be Star-Forming in the optics. In the text we analyze the consequence to change their AGN flag to 0. 
\label{litt_sample_ref}}
\tablehead{
\colhead{Name} &
\colhead{$\log(M_\ast/M_\odot)$} &
\colhead{AGN} &
\colhead{Refs} 
}
\def\arraystretch{2}
\startdata
\hline
  MIP001417-302303 & 9.6 [\cite{rawle+2014}] & 0 [\cite{owers+2012}] & \cite{owers+2012}, \cite{rawle+2014}\\
  HLS001427-302344 & 10.9 [\cite{rawle+2014})] & 1 [\cite{owers+2012})] & \cite{owers+2012}, \cite{rawle+2014}\\ 
  NGC1566 & 10.8 [\cite{elagali+2019}] & 1 [\cite{veron+2006}] & \cite{elagali+2019}\\
  ID345 & 10.3 [\cite{boselli+2019}] & 1 [\cite{boselli+2019}] & \cite{boselli+2019}\\
  LEDA36382 & 9.5 [\cite{mendel+2014}] & 0 [\cite{sdss}] & \cite{gavazzi+1995}, \cite{gavazzi+2001}, \cite{sivanandam+2014}, \cite{boselli+2018}, \cite{yagi+2017} \\
  UGC6697 & 9.8 [\cite{yagi+2017}] & 0 [\cite{consolandi+2017}] & \cite{gavazzi+1984}, \cite{gavazzi+1989}, \cite{gavazzi+1995},\cite{gavazzi+2001}, \cite{scott+2010}, \cite{fruscione+1990}, \cite{sun+2005}, \cite{yagi+2017}, \cite{consolandi+2017}\\
  2MASXJ11443212+2006238 & 9.9  [\cite{yagi+2017}] & 0  [\cite{sdss}] & \cite{gavazzi+1989}, \cite{gavazzi+1995}, \cite{gavazzi+2001}, \cite{yagi+2017}, \cite{gavazzi+2017}\\
  NGC4254 & 10.1 [\cite{boselli+2018}] & 2 [\cite{davies+2020}] & \cite{boselli+2018}, \cite{wezgowiec+2012}, \cite{chyzy+2007}, \cite{kantharia+2008},  \cite{rahman+2011}\\
  NGC4388 & 9.9 [\cite{boselli+2015}] & 2 [\cite{boselli+2015}] & \cite{vollmer+2003}, \cite{vollmer+2009}, \cite{oosterlo+2005}, \cite{chung+2009}, \cite{yoshida+2004}, \cite{yoshida+2002}, \cite{yagi+2013}, \cite{gu+2013},\cite{damas+2016}\\
  NGC4402 & 10.0 [\cite{boselli+2015}] & 0 [\cite{decarli+2007}] &  \cite{lee+2017}, \cite{abramson+2014}, \cite{cramer+2020}, \cite{abramson+2016}\\
  NGC4424 & 10.2 [\cite{boselli+2015}]  & 0 [\cite{filippenko+1997}] & \cite{chung+2007}\\
  NGC4438 & 10.4 [\cite{boselli+2015}] & 3 [\cite{veron+2003}] & \cite{boselli+2005}, \cite{vollmer+2009}, \cite{wang+2020}, \cite{kenney+1995}, \cite{chemin+2005}, \cite{kenney+2008}\\
  IC3418 & 8.4 [\cite{boselli+2015}] & 0 [\cite{fumagalli+2011}] & \cite{hester+2010}, \cite{fumagalli+2011}, \cite{kenney+2014}\\
  NGC4501 & 10.7 [\cite{boselli+2015}] & 2 [\cite{boselli+2015}] & --\\
  NGC4522 & 9.1 [\cite{boselli+2015}] & 0 [\cite{sdss}] & \cite{kenney+2004}, \cite{abramson+2016}, \cite{lee+2018}, \cite{minchin+2019}, \cite{stein+2017}, \cite{vollmer+2004}\\
  NGC4548 & 10.5 [\cite{boselli+2015}] & 3 [\cite{boselli+2015}] & --\\
  NGC4569 & 10.4 [\cite{boselli+2015}] & 3  [\cite{boselli+2015}] & \cite{boselli+2016}, \cite{boselli+2006}, \cite{tschoke+2001}, \cite{vollmer+2004}, \cite{wezgowiec+2012}\\
  GMP6364 & 8.5 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP5821 & 8.9 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  IC3913 & 11.0 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{salim+2018}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP5382 & 9.3 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP4688 & 8.5 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP4629 & 8.6 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{salim+2018}, \cite{chen+2020}, \cite{roberts+2020}, \cite{gavazzi+2018}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP4570 & 8.1 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{salim+2018}, \cite{chen+2020}, \cite{roberts+2020}, \cite{gavazzi+2018}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP4555 & 9.9 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{salim+2018}, \cite{chen+2020}, \cite{salim+2018}, \cite{salim+2016}, \cite{gavazzi+2018}\\
  MACSJ1258-JFG1 & 10.5 (*) & 1 [\cite{rakshit+2017}] & \cite{ebeling+2014}, \cite{mcpartland+2016}\\
  NGC4848 & 10.8 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{chen+2020}, \cite{salim+2018}, \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}, \cite{fossati+2012}, \cite{yagi+2013}, \cite{gavazzi+2018}\\
  GMP4437 & 10.4 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP4463 & 9.3 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP4281 & 9.7 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP4236 & 8.4 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  NGC4853 & 10.8  [\cite{salim+2016}] & 2 [\cite{mahajan+2010}] & \cite{yagi+2010}, \cite{salim+2018}, \cite{salim+2016}, \cite{chen+2020}, \cite{gavazzi+2018}\\
  GMP4159 & 9.8 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP4135 & 9.8 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP4106 & 9.1 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  IC3949 & 10.6 [\cite{salim+2016}] & 2 [\cite{mahajan+2010}] & \cite{yagi+2010}, \cite{chen+2020}, \cite{gavazzi+2018}, \cite{salim+2018}, \cite{salim+2016}\\
  NGC4858 & 10.2 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{chen+2020}, \cite{yagi+2010}, \cite{salim+2018}, \cite{roberts+2020}, \cite{gavazzi+2018}, \cite{salim+2018}, \cite{salim+2016}\\
  Mrk58 & 9.8 [\cite{salim+2016}] & 0 [\cite{sdss}] &\cite{chen+2020}, \cite{yagi+2010}, \cite{roberts+2020}, \cite{gavazzi+2018}, \cite{salim+2018}, \cite{salim+2016} \\
  GMP3618 & 10.1 [\cite{salim+2016}] & 6 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP3271 & 9.1 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{yagi+2010}, \cite{chen+2020}, \cite{roberts+2020}, \cite{gavazzi+2018}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP3253 & 9.4 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP3143 & 8.9 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP3071 & 9.3 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{chen+2020}, \cite{roberts+2020}, \cite{yagi+2010}, \cite{yoshida+2012}\\
  SDSSJ130006.15+281507.8 & 8.8 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  D100 & 9.3 [\cite{salim+2016}] & 2 [\cite{mahajan+2010}] & \cite{chen+2020}, \cite{yagi+2010}, \cite{smith+2010}, \cite{jachym+2017}, \cite{roberts+2020}, \cite{cramer+2019}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP2625 & 9.1 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP2599 & 9.9 [\cite{salim+2016}] & 4 [\cite{nucita+2017}, \cite{birchall+2020}] & \cite{chen+2020}, \cite{smith+2010}, \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  IC4040 & 10.3 [\cite{salim+2016}] & 5 [\cite{best+2012}] & \cite{chen+2020}, \cite{smith+2010}, \cite{yagi+2010}, \cite{yoshida+2012}, \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  NGC4911 & 11.3 [\cite{salim+2016}] & 2 [\cite{mahajan+2010}] & \cite{chen+2020}, \cite{yagi+2010}, \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016} \\
  GMP2073 & 10.4 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  NGC4921 & 11.0 [\cite{salim+2016}] & 6 [\cite{mahajan+2010}] & \cite{kenney+2015}, \cite{chen+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP1616 & 10.3 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP1582 & 8.7 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP713 & 9.0 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP672 & 8.7 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP597 & 8.7 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP522 & 9.9 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP455 & 9.4 [\cite{salim+2016}] & 0 [\cite{mahajan+2010}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP406 & 9.0 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  GMP223 & 8.5 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  SDSSJ130545.34+285216.8 & 9.2 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  SDSSJ130553.48+280644.7 & 10.1 [\cite{salim+2016}] & 0 [\cite{sdss}] & \cite{roberts+2020}, \cite{salim+2018}, \cite{salim+2016}\\
  JO147 & 10.8 [\cite{merluzzi+2010}] & 3  & \cite{merluzzi+2013}, \cite{merluzzi+2016}, \cite{gullieuszik+2020}\\
  SOS90630 & 10.0 [\cite{merluzzi+2016}] & 0 [\cite{merluzzi+2016}] & \cite{merluzzi+2016}\\
  SOS61086 & 9.6 [\cite{merluzzi+2016}] & 0 [\cite{merluzzi+2016}] & \cite{merluzzi+2016}\\
  d4 & 9.8 [\cite{ebeling+2019}] & 0 [\cite{ebeling+2019}] & \cite{ebeling+2019}\\
  A1758N\_JFG1 & 10.9 [\cite{ebeling+2019}] & 0 [\cite{kalita+2019}] & \cite{ebeling+2019}\\
  d5 & 10.1 [\cite{ebeling+2019}] & 0 [\cite{ebeling+2019}] & \cite{ebeling+2019}\\
  d7 & 9.8 [\cite{ebeling+2019}] & 4 [\cite{ebeling+2019}] & \cite{ebeling+2019}\\
  d6 & 8.9 [\cite{ebeling+2019}] & 0 [\cite{ebeling+2019}] & \cite{ebeling+2019}\\
  d3 & 8.4 [\cite{ebeling+2019}] & 0 [\cite{ebeling+2019}] & \cite{ebeling+2019}\\
  d1 & 8.5 [\cite{ebeling+2019}] & 0 [\cite{ebeling+2019}] & \cite{ebeling+2019}\\
  d2 & 9.5 [\cite{ebeling+2019}] & 0 [\cite{ebeling+2019}] & \cite{ebeling+2019}\\
  C153 & 10.4 (*) & 3 [\cite{owen+2006}] & \cite{owen+2006}\\
  ESO137-001 & 9.6 [\cite{sun+2010}] & 0 [\cite{fossati+2016}] & \cite{sun+2010}, \cite{sun+2006}, \cite{sun+2007}, \cite{sun+2010}, \cite{sivandam+2010}, \cite{jachym+2019}, \cite{jachym+2014}, \cite{fossati+2016}, \cite{fumagalli+2014}, \cite{zhang+2013}\\
  ESO137-002 & 10.3 [\cite{sun+2010}] & 4 [\cite{sun+2010}] & \cite{zhang+2013}, \cite{ruszkowski+2014}, \cite{sun+2007}\\
  Sausage9 & 10.6 [\cite{sobral+2015}] & 2 [\cite{sobral+2015}] & \cite{stroe+2020}\\
  Sausage7 & 10.5 [\cite{sobral+2015}] & 0 [\cite{sobral+2015}] & \cite{stroe+2020}\\
  Sausage6 & 9.4 [\cite{sobral+2015}] & 0 [\cite{sobral+2015}] & \cite{stroe+2020}\\
  Sausage8 & 10.6 [\cite{sobral+2015}] & 2 [\cite{sobral+2015}] & \cite{stroe+2020}\\
  Sausage5 & 9.6 [\cite{sobral+2015}] & 0 [\cite{sobral+2015})] & \cite{stroe+2020}\\
  235144-260358 & 9.3 (*) & 0 [\cite{cortese+2007}] &\cite{cortese+2007}\\
\hline
\enddata
\end{deluxetable*}




==> AASTeX Template for submissions to AAS Journals (ApJ-AJ-ApJS-ApJL-PSJ-RN) (2) (4)/table4_short.tex <==

\begin{table*}
\begin{center}
\caption{Columns are 1) galaxy name 2) logarithm of the stellar masses, adopting  Chabrier 2003 IMF (in parenthesis the reference from which the value has been taken is reported) 3) AGN classification (see Table \ref{gasp_agn}) and relative reference 4) references which present a characterization of the galaxy as a RPS candidate. The four galaxies with classification equals to 4 and 5 (e.g. where the AGN is spotted observing them in X and radio) resulted to be Star-Forming in the optics. In the text we analyze the consequence to change their AGN flag to 0. 
\label{litt_sample_ref}} 
\scriptsize
\begin{tabular}{cccc}
%%%\tablehead{
%%%  \colhead{name} &
%%%  \colhead{RA} &
%%%  \colhead{DEC} &
%%%  \colhead{z} &
%%%  \colhead{cluster} &
%%%  \colhead{Jstage} &
%%%  \colhead{Jstage$_{\rm gen}$} &
%%%  \colhead{comments}
%%% }
\hline
\hline
name & $\log(M_\ast/M_\odot)$ & AGN & Refs  \\
\hline
  MIP001417-302303 & 9.6 [\cite{rawle+2014}] & 0 [\cite{owers+2012}] & \cite{owers+2012}, \cite{rawle+2014}\\
  HLS001427-302344 & 10.9 [\cite{rawle+2014})] & 1 [\cite{owers+2012})] & \cite{owers+2012}, \cite{rawle+2014}\\ 
  NGC1566 & 10.8 [\cite{elagali+2019}] & 1 [\cite{veron+2006}] & \cite{elagali+2019}\\
  ID345 & 10.3 [\cite{boselli+2019}] & 1 [\cite{boselli+2019}] & \cite{boselli+2019}\\
  \multirow{2}{*}{LEDA36382} & \multirow{2}{*}{9.5 [\cite{mendel+2014}]} & \multirow{2}{*}{0 [\cite{sdss}]} & \cite{gavazzi+1995}, \cite{gavazzi+2001},\\
  &&& \cite{sivanandam+2014}, \cite{boselli+2018}, \cite{yagi+2017} \\
\hline
\end{tabular}%
\end{center}
\tablecomments{This table is published in its entirety in machine-readable format.  A portion is shown here for guidance regarding its form and content.}\end{table*}



==> table3_ALL_revised.tex <==
\begin{longrotatetable}
\begin{deluxetable}{ccccccccc}
\tabletypesize{\tiny}
\tablecaption{Colums are: 1) name 2) and 3) equatorial coordinates of the galaxy center from SIMBAD 4) galaxy redshift 5) host cluster 6) and 7) Jstage and general Jstage, defined in section \S3.2 8) alternative names and authors from which information have been taken. Stellar masses flagged with the asterisk (*) are computed by means of photometric data as described in Sec.\ref{sec:appendix_mass}. 
\label{litt_sample}}
\tablehead{
  \colhead{name} &
  \colhead{RA} &
  \colhead{DEC} &
  \colhead{z} &
  \colhead{cluster} &
  \colhead{Jstage} &
  \colhead{Jstage$_{\rm gen}$} &
  \colhead{comments}
 }
 \tablewidth{0pt}
  \startdata
\hline
  MIP001417-302303 & 3.5693 & -30.3843 & 0.2955 & A2744 & -- & 2.0 & F1228\\
  HLS001427-302344 & 3.61065 & -30.39581 & 0.3033 & A2744 & -- & 2.0 & F0083\\
  NGC1566 & 65.00175 & -54.93781 & 0.005 & Dorado & 0.0 & 0.0 & --\\
  ID345 & 149.9191 & 2.5281 & 0.727 & CGr32 & 2.0 & 2.0 & --\\
  LEDA36382 & 175.73523 & 19.96621 & 0.02427 & A1367 & 2.0 & 2.0 & CGCG97073\\
  UGC6697 & 175.95446 & 19.96844 & 0.02243 & A1367 & 2.0 & 2.0 & CGCG097-087\\
  2MASXJ11443212+2006238 & 176.13385 & 20.10662 & 0.02398 & A1367 & 2.0 & 2.0 & --\\
  NGC4254 & 184.70668 & 14.41651 & 0.00803 & Virgo & 1.0 & 2.0 & MESSIER099\\
  NGC4388 & 186.44508 & 12.66207 & 0.00856 & Virgo & 1.0 & 2.0 & UGC07520, VCC 0836, VPC 0438, CGCG070068\\
  NGC4402 & 186.53189 & 13.11332 & 0.0008   & Virgo & 3.0 & 0.5 &   VCC873\\    
  NGC4424 & 186.79838 & 9.42067  & 0.0015 & Virgo & 0.5 & 2             & -- \\
  NGC4438 & 186.93997 & 13.00883 & 0.0003 & Virgo & -- & -- & --\\
  IC3418 & 187.43301 & 11.40469 & 0.00013 & Virgo & 0.5 & 2.0 & VCC1217\\
  NGC4501 & 187.9965 & 14.42039 & 0.00761 & Virgo & -- & 0.5 & MESSIER088\\
  NGC4522 & 188.41546 & 9.17502 & 0.0077 & Virgo & 3.0 & 1.0 & --\\
  NGC4548 & 188.86022 & 14.49634 & 0.00164 & Virgo & 0.0 & 0.0 & MESSIER091\\
  NGC4569 & 189.20747 & 13.16294 & 0.0008.0 & Virgo & 2.0 & 2.0 & MESSIER090, UGC07786, VCC 1690\\
  GMP6364 & 193.67526 & 27.63897 & 0.02874 & Coma & -- & 2.0 & SDSS J125442.05+273820.2\\
  GMP5821 & 193.93454 & 28.75464 & 0.0275 & Coma & -- & -- & SDSS J125544.29+284516.6\\
  IC3913 & 194.11905 & 27.29128 & 0.0251 & Coma & -- & -- & GMP5422, KUG 1254+275, CGCG160026\\
  GMP5382 & 194.11967 & 29.13708 & 0.03163 & Coma & -- & 0.0 & 2MASX J12562871+2908140, SDSS J125628.71+290813.5\\
  GMP4688 & 194.43215 & 29.00331 & 0.0231 & Coma & -- & 1.0 & LEDA 1852727\\
  GMP4629 & 194.4593 & 28.17036 & 0.0231 & Coma & 1.0 & 1.0 & SDSSJ125750.2+281013\\
  GMP4570 & 194.48665 & 27.99176 & 0.0152 & Coma & 2.0 & 2.0 & SDSSJ125756.79+275930\\
  GMP4555 & 194.4905 & 28.06178 & 0.0271 & Coma & 2.0 & 2.0 & SDSSJ125757.7+280342, KUG1255+283\\
  MACSJ1258-JFG1 & 194.49833 & 47.0461 & 0.3424 & MACSJ1258.0+4702 & -- & 2.0 & --\\
  NGC4848 & 194.52352 & 28.24274 & 0.0314 & Coma & 2.0 & 2.0 & GMP4471, CGCG 160-055, SDSSJ125805.6+281433, UGC08082, KUG 1255+285\\
  GMP4437 & 194.53846 & 28.70859 & 0.0254 & Coma & -- & 0.0 & --\\
  GMP4463 & 194.53858 & 26.66409 & 0.0243 & Coma & -- & 0.0 & --\\
  GMP4281 & 194.60575 & 28.12897 & 0.0274 & Coma & -- & 0.0 & --\\
  GMP4236 & 194.6285 & 26.99494 & 0.0249 & Coma & -- & 1.0 & --\\
  NGC4853 & 194.64663 & 27.59633 & 0.0256 & Coma & 0.0 & 0.0 & --\\
  GMP4159 & 194.64717 & 27.26486 & 0.0245 & Coma & -- & 0.5 & SDSSJ125835.2+273547, GMP4156, CGCG160068,  UGC08092, KUG1256+278B, D43\\
  GMP4135 & 194.65538 & 27.17625 & 0.0256 & Coma & -- & 1.0 & Mrk 56, KUG1256+27\\
  GMP4106 & 194.66637 & 26.7595 & 0.0249 & Coma & -- & 1.0 & Mrk057, KUG1256+274\\
  IC3949 & 194.73338 & 27.83336 & 0.0253 & Coma & 1.0 & 1.0 & --\\
  NGC4858 & 194.7585 & 28.11575 & 0.0314 & Coma & 2.0 & 2.0 &  SDSSJ125856.0+275000, GMP3896, CGCG160212, UGC08096, D89\\
  Mrk58 & 194.772 & 27.64446 & 0.0181 & Coma & 2.0 & 2.0 & GMP3816, SDSSJ125902.0+280656, CGCG160213, KUG1256+283\\
  GMP3618 & 194.81937 & 27.10608 & 0.028 & Coma & -- & 0.5 & GMP3779, KUG1256+279, CGCG160073, SDSSJ125905.2+27383840, D54, RB219\\
  GMP3271 & 194.91621 & 27.57625 & 0.0167 & Coma & 0.5 & 1.0 & --\\
  GMP3253 & 194.91721 & 28.63081 & 0.0178 & Coma & -- & 0.5 & D41, SDSSJ125939.8+273435, KUG1257+278\\
  GMP3143 & 194.95524 & 26.97433 & 0.0235 & Coma & -- & 0.0 & KUG 1257+288B\\
  GMP3071 & 194.9838 & 27.74633 & 0.0298 & Coma & 2.0 & 2.0 & --\\
  SDSSJ130006.15+281507.8 & 195.02568 & 28.25234 & 0.0212 & Coma & -- & 2.0 & --\\
  D100 & 195.03809 & 27.86649 & 0.0177 & Coma & 2.0 & 2.0 & Mrk60, GMP2910\\
  GMP2625 & 195.13003 & 28.95054 & 0.0233 & Coma & -- & 0.5 & --\\
  GMP2599 & 195.14031 & 27.63777 & 0.025 & Coma & 0.0 & 1.0 & --\\
  IC4040 & 195.15777 & 28.05809 & 0.0255 & Coma & 2.0 & 2.0 & KUG1258+279A, 7W 1258+27W06\\
  NGC4911 & 195.23357 & 27.79087 & 0.0266 & Coma & 1.0 & 1.0 & --\\
  GMP2073 & 195.35448 & 28.67723 & 0.0292 & Coma & -- & 0.0 & GMP2374\\
  NGC4921 & 195.35884 & 27.886 & 0.0183 & Coma & 0.0 & 0.0 & --\\
  GMP1616 & 195.53284 & 27.64831 & 0.023 & Coma & -- & 0.0 & GMP2059\\
  GMP1582 & 195.54739 & 28.17326 & 0.0299 & Coma & -- & 0.0 & --\\
  GMP713 & 195.97679 & 28.31054 & 0.0268 & Coma & -- & -- & LEDA 83761\\
  GMP672 & 195.98809 & 26.72948 & 0.022 & Coma & -- & 1.0 & --\\
  GMP597 & 196.0547 & 28.54245 & 0.0271 & Coma & -- & 0.5 & --\\
  GMP522 & 196.09452 & 28.81077 & 0.0265 & Coma & -- & 1.0 & --\\
  GMP455 & 196.11063 & 27.30431 & 0.0184 & Coma & -- & 2.0 & --\\
  GMP406 & 196.16159 & 28.97269 & 0.0253 & Coma & -- & 0.0 & --\\
  GMP223 & 196.27764 & 28.64115 & 0.0182 & Coma & -- & 1.0 & --\\
  SDSSJ130545.34+285216.8 & 196.439 & 28.87133 & 0.0266 & Coma & -- & 1.0 & --\\
  SDSSJ130553.48+280644.7 & 196.47287 & 28.11244 & 0.0246 & Coma & -- & 0.0 & --\\
  JO147 & 201.707304 & -31.39575 & 0.0506 & A3558 & 2.0 & 2.0 & SOS114372\\
  SOS90630 & 202.368875 & -31.657111 & 0.049 & SC1327-312 & 2.0 & 2.0 & --\\
  SOS61086 & 202.999167 & -31.822833 & 0.045 & SC1329-313 & 2.0 & 2.0 & --\\
  d4 & 203.135758 & 50.564581 & 0.272 & A1758 & -- & 0.5 & --\\
  A1758N\_JFG1 & 203.146583 & 50.52675 & 0.2733 & A1758 & 0.0 & 1.0 & --\\
  d5 & 203.17445 & 50.525994 & 0.2716 & A1758 & -- & 0.5 & --\\
  d7 & 203.184258 & 50.518794 & 0.2875 & A1758 & -- & 0.0 & --\\
  d6 & 203.1906 & 50.527164 & 0.2668 & A1758 & -- & 0.5 & --\\
  d3 & 203.208908 & 50.555894 & 0.2755 & A1758 & -- & 1.0 & --\\
  d1 & 203.224104 & 50.526292 & 0.2686 & A1758 & -- & 2.0 & --\\
  d2 & 203.226979 & 50.516425 & 0.2719 & A1758 & -- & 1.0 & --\\
  C153 & 235.2875 & 66.26222 & 0.2525 & A2125 & -- & 1.0 & --\\
  ESO137-001 & 243.363771 & -60.764053 & 0.01557 & A3627 & 2.0 & 2.0 & --\\
  ESO137-002 & 243.398546 & -60.865167 & 0.0191 & A3627 & 2.0 & 2.0 & --\\
  Sausage9 & 340.671125 & 52.974631 & 0.1839 & CIZAJ2242.8+5301 & -- & -- & --\\
  Sausage7 & 340.740125 & 53.087431 & 0.1832 & CIZAJ2242.8+5301 & -- & -- & --\\
  Sausage6 & 340.749375 & 53.037381 & 0.1836 & CIZAJ2242.8+5301 & -- & -- & --\\
  Sausage8 & 340.787 & 53.090289 & 0.1843 & CIZAJ2242.8+5301 & -- & -- & --\\
  Sausage5 & 340.80375 & 53.0028 & 0.1825 & CIZAJ2242.8+5301 & -- & -- & --\\
  235144-260358 & 357.933458 & -26.066555 & 0.2265 & A2667 & -- & 2.0 & --\\
\enddata
\end{deluxetable}
\end{longrotatetable}



